A Scalable Auxiliary Space Preconditioner for High-Order Finite Element Methods

In this paper, we revisit an auxiliary space preconditioning method proposed by Xu [Computing 56, 1996], in which low-order finite element spaces are employed as auxiliary spaces for solving linear algebraic systems arising from high-order finite element discretizations. We provide a new convergence rate estimate and parallel implementation of the proposed algorithm. We show that this method is user-friendly and can play an important role in a variety of Poisson-based solvers for more challenging problems such as the Navier--Stokes equation. We investigate the performance of the proposed algorithm using the Poisson equation and the Stokes equation on 3D unstructured grids. Numerical results demonstrate the advantages of the proposed algorithm in terms of efficiency, robustness, and parallel scalability.

==> precond.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Diagonal and triangular preconditioners for saddle point problems}\label{sec:precond}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we discuss how to solve the discrete saddle point problem arising from the mixed finite element discretization of the system \eqref{pde1}--\eqref{pde3} iteratively. Let the coefficient matrix
\[
K :=
 \left ( \begin{array}{cc} \alpha M_\vu + A & B^T \\ B & 0 \end{array}
 \right),
\]
where $B$ is simply the discrete divergence operator $-\nabla_h\cdot$, $A$ and $M_\vu$ are block diagonal matrices with the discrete Laplace operator $-\Delta_h$ and velocity mass matrices on their diagonal, respectively. We need to solve the system of linear equations
\begin{equation}\label{saddlepoint}
K \left[ \begin{array}{c} \vu \\ p \end{array} \right] =  \left[ \begin{array}{c} \vf \\ g \end{array} \right].
\end{equation}
Notice that $\vu$ and $p$ are vectors at degrees of freedom of the velocity field and pressure, respectively. Without raising any confusion, we will use the same notation as the functions. 

As K is a symmetric positive semidefinite matrix, 
we apply Krylov iterative methods for indefinite problems. For example, we
can use minimal residual (MinRes) method or generalized minimal residual (GMRes) method. The minimal residual method for general indefinite system has been
studied by Paige and Saunders and Chandra. As analyzed in [ ], the convergence rate of minimal residual method is governed by three parameters: the conditioning of A and B and the relative scaling between them. However, as here
$\text{cond}(A)=O(h^{-2})$, a direct application of minimal residual method
is not practical, as the convergence rate will be too slow. Then we
will find a good preconditioner for this method, that's instead of
solving $Kx=b$ directly, we will solve the left preconditioned system $QKx=Qb$ with Krylov methods. We only consider a symmetric diagonal preconditioner for MinRes method and an upper triangular preconditioner for GMRes method here in this paper. 

Using a block triangular factorization of $K$, we can write 
\[
K = 
%
\left(
\begin{array}{cc}
I_\vu & 0 \\
B(\alpha M_\vu + A)^{-1} & I_p 
\end{array}
\right)
%
\left(
\begin{array}{cc}
\alpha M_\vu + A & B^T \\
0 & -B(\alpha M_\vu + A)^{-1}B^T 
\end{array}
\right).
\]
Note that forming such a factorization is as expensive as solving the original system. But it motives a block upper triangular preconditioner 
\begin{equation}\label{precond_t}
Q_t =
\left (
\begin{array}{cc} \alpha M_\vu + A & B^T \\ 0 & -S \end{array}
\right)^{-1}
\end{equation}
or, simply, a block diagonal preconditioner
\begin{equation}\label{precond_d}
Q_d =
\left (
\begin{array}{cc} \alpha M_\vu + A & 0 \\ 0 & -S \end{array}
\right)^{-1},
\end{equation}
where $S$ is an approximation of the Schur complement $B(\alpha M_\vu + A)^{-1}B^T$. Bramble and Pasciak~\cite{1988,Bramble.J;Pasciak.J1997}

We can form an approximation to $(\alpha M_\vu + A)^{-1}$ by applying one AMG V-cycle to $\alpha \diag(M_\vu) + A$. As for the Schur complement part, $S^{-1}$ can be approximated by $M_p + \alpha(-\Delta_N)^{-1}$, where $M_p$ is the pressure mass matrix and $-\Delta_N$ is the auxiliary discrete Laplace operator  with the Neumann boundary condition on $P^{k-1,0}$ space. 

